Ensemble prosody prediction for expressive speech synthesis

Generating expressive speech with rich and varied prosody continues to be a challenge for Text-to-Speech. Most efforts have focused on sophisticated neural architectures intended to better model the data distribution. Yet, in evaluations it is generally found that no single model is preferred for all input texts. This suggests an approach that has rarely been used before for Text-to-Speech: an ensemble of models. We apply ensemble learning to prosody prediction. We construct simple ensembles of prosody predictors by varying either model architecture or model parameter values. To automatically select amongst the models in the ensemble when performing Text-to-Speech, we propose a novel, and computationally trivial, variance-based criterion. We demonstrate that even a small ensemble of prosody predictors yields useful diversity, which, combined with the proposed selection criterion, outperforms any individual model from the ensemble.

==> figures/archive.tex <==
% TABLES
% TABLES

% \begin{figure}[htb]
%   \centering
%     \centerline{\includegraphics[width=8.5cm]{figures/tmp/accuracy.png}}
%     \caption{Accuracy of crowd wisdom, single models and ensemble selection. $^{\star}$ denotes accuracy rates that are statistically significantly above random chance.}
%     \label{fig:accuracy}
% \end{figure}

% \begin{figure}[htb]
%   \centering
%     \centerline{\includegraphics[width=8.5cm]{figures/tmp/keywords.png}}
%     \caption{Frequency of keywords tagged in free-text descriptions of perceived ensemble diversity. The total number of comments received are in brackets next to each ensemble}
%     \label{fig:diversity}
% \end{figure}


% INTRO ARCHIVE
% Ensembling is a widely used technique in prediction and generation tasks. It is used as a method to estimate and reduce uncertainty [citation], detect distribution shifts [citation], increase prediction accuracy [citation], and to generate variety [citation], which is our primary interest in this work. In principle, generative models can model the distribution of the data, and facilitate the generation of new samples from that learnt distribution. However, in practice, given the multi-faceted and probabilistic nature of prosody, different models can end up learning different aspects of the distribution, influenced by inductive bias and randomness, that are difficult to perfectly distill into a single model. 

% There are two inference methods in ensembling - prediction and selection. Ensemble prediction combines the output of multiple models in an additive or multiplicative manner, in order to form the final prediction; ensemble selection generates multiple outputs, ranks them by some criteria, then selects one as the output. In this paper, we adopt ensemble selection, as we wish to mitigate the ``average prosody" effect from maximum likelihood-based training. Conceptually, the ensemble prediction approach, if applied directly to prosody prediction, is likely to exacerbate the averaging effect.

% TTS ensemble selection requires the ensemble to be able to generate diverse renditions of the same utterance, and the ability to automatically identify the more expressive rendition. 


% LIT REVIEW
% **************
% ***** GV *****
% **************
% 1. SPECTRAL CONVERSION BASED ON MAXIMUM LIKELIHOOD ESTIMATION
% CONSIDERING GLOBAL VARIANCE OF CONVERTED PARAMETER (ICASSP 2005)
% - https://www.cs.cmu.edu/~awb/papers/icassp2005/0100009.pdf
% - Abstract: 
%     This paper describes a novel spectral conversion method for the
%     voice transformation. We perform spectral conversion between
%     speakers using a Gaussian Mixture Model (GMM) on joint probability density of source and target features. A smooth spectral sequence can be estimated by applying maximum likelihood (ML)
%     estimation using dynamic features to the GMM-based mapping.
%     However, the degradation of the converted speech quality is still
%     caused due to an over-smoothing of the converted spectra, which
%     is inevitable in the conventional ML-based parameter estimation.
%     In order to alleviate the over-smoothing, we propose an ML-based
%     conversion taking account of the global variance of the converted
%     parameter in each utterance. Experimental results show that the
%     performance of the voice conversion can be improved by using the
%     global variance information. Moreover, it is demonstrated that the
%     proposed algorithm is more effective than spectral enhancement
%     by postfiltering.
% - Notes: First appearance of GV (only spectral parameters), applied to voice conversion (F0 obtained from ref).

% 2. Speech Parameter Generation Algorithm Considering Global Variance for HMM-Based Speech (Interspeech 2005)
% - https://citeseerx.ist.psu.edu/viewdoc/download?doi=10.1.1.210.5031&rep=rep1&type=pdf
% - Abstract: 
%     This paper describes a novel parameter generation algorithm for the HMM-based speech synthesis. The conventional algorithm generates a trajectory of static features that maximizes an output probability of a parameter sequence consisting of the static and dynamic features from HMMs under an actual constraint between the two features. The generated trajectory is often excessively smoothed due to the statistical processing. Using the over-smoothed trajectory causes the muffled sound. In order to alleviate the over-smoothing effect, we propose the generation algorithm considering not only the output probability used for
%     the conventional method but also that of a global variance (GV) of the generated trajectory. The latter probability works as a penalty for a reduction of the variance of the generated trajectory. A result of a perceptual evaluation demonstrates that the proposed method causes large improvements of the naturalness of synthetic speech.
% - Snippets: 
%     - considering GV to not only spectral parameter generation but also F0 parameter generation in the HMM-based speech synthesis.
%     - As a spectral parameter, we used 0th through 24th melcepstral coefficients obtained from the smoothed spectrum analyzed by STRAIGHT [10]. As a source parameter, we used a log-scaled F0 automatically extracted from a waveform
%     - In the results, GV actually seemed way more impactful than F0

% 3. Modeling of Speech Parameter Sequence Considering Global Variance for HMM-Based Speech Synthesis (Book chapter, 2010)
% - https://www.intechopen.com/chapters/15360
% - snippets:
%     - GV penalty applied in training the spectral and F0 components
%     - As one of the most effective features for capturing properties not
%     well modeled by traditional HMMs, Toda and Tokuda (Toda & Tokuda (2007)) proposed
%     the global variance (GV), which is the variance of the static feature vectors calculated over
%     a time sequence (e.g., over an utterance). It has been found that the GV is inversely correlated
%     with the oversmoothing effect. Therefore, a metric on the GV of the generated parameters
%     effectively acts as a penalty term in the parameter generation process. Several papers (Toda
%     & Tokuda (2007); Zen et al. (2007a; 2008)) have reported that the naturalness of synthetic
%     speech is significantly improved by considering the GV in HMM-based speech synthesis.
%     Moreover, it has been reported that the use of the GV is also effective for improving other
%     statistical parametric speech synthesis techniques such as voice conversion (Toda et al. (2007)).
%     It is not an exaggeration to say that GV modeling has significantly contributed to the recent
%     improvements in those techniques.
% - Notes: 
%     - HMM synthesis: GV on spectral features from MFCC and F0 components from waveform

% **************
% ***** F0 *****
% **************
% 1. Perception of prosodic variation for speech synthesis using an unsupervised discrete representation of F0 (Zack's paper, SP2020)
% - https://arxiv.org/abs/2003.06686
% % - Abstract:
% %     In English, prosody adds a broad range of information to segment sequences, from information structure (e.g. contrast) to stylistic variation (e.g. expression of emotion). However, when learning to control prosody in text-to-speech voices, it is not clear what exactly the control is modifying. Existing research on discrete representation learning for prosody has demonstrated high naturalness, but no analysis has been performed on what these representations capture, or if they can generate meaningfully-distinct variants of an utterance. We present a phrase-level variational autoencoder with a multi-modal prior, using the mode centres as "intonation codes". Our evaluation establishes which intonation codes are perceptually distinct, finding that the intonation codes from our multi-modal latent model were significantly more distinct than a baseline using k-means clustering. We carry out a follow-up qualitative study to determine what information the codes are carrying. Most commonly, listeners commented on the intonation codes having a statement or question style. However, many other affect-related styles were also reported, including: emotional, uncertain, surprised, sarcastic, passive aggressive, and upset.

% 2. Using generative modelling to produce varied intonation for speech synthesis (Also Zack's paper, SSW2019)
% - https://arxiv.org/abs/1906.04233
% % - Abstract:
% %     Unlike human speakers, typical text-to-speech (TTS) systems are unable to produce multiple distinct renditions of a given sentence. This has previously been addressed by adding explicit external control. In contrast, generative models are able to capture a distribution over multiple renditions and thus produce varied renditions using sampling. Typical neural TTS models learn the average of the data because they minimise mean squared error. In the context of prosody, taking the average produces flatter, more boring speech: an "average prosody". A generative model that can synthesise multiple prosodies will, by design, not model average prosody. We use variational autoencoders (VAEs) which explicitly place the most "average" data close to the mean of the Gaussian prior. We propose that by moving towards the tails of the prior distribution, the model will transition towards generating more idiosyncratic, varied renditions. Focusing here on intonation, we investigate the trade-off between naturalness and intonation variation and find that typical acoustic models can either be natural, or varied, but not both. However, sampling from the tails of the VAE prior produces much more varied intonation than the traditional approaches, whilst maintaining the same level of naturalness.

% 3. A Vector Quantized Variational Autoencoder (VQ-VAE) Autoregressive Neural F0 Model for Statistical Parametric Speech Synthesis
% - https://ieeexplore.ieee.org/document/8884734


% ***************
% ***** ASR *****
% ***************
% 1. Ensemble Deep Learning for Speech Recognition
% https://www.microsoft.com/en-us/research/wp-content/uploads/2016/02/EnsembleDL_submitted.pdf
% - Snippets:
%     - linear and log-linear stacking methods for ensemble learning with applications specifically to speech class posterior probabilities as computed by the convolutional, recurrent, and fully-connected deep neural networks.

% 2. Mark's slides 
% http://mi.eng.cam.ac.uk/~mjfg/mjfg_tcstar.pdf



% ***************
% ** ENSEMBLES **
% ***************
% 1. Token-Level Ensemble Distillation for Grapheme-to-Phoneme Conversion (INTERSPEECH 2019)
% https://arxiv.org/pdf/1904.03446.pdf
% - Snippets:
%     - token-level ensemble knowledge distillation to boost the accuracy of G2P conversion
%     - Model ensemble can incorporate the advantages of individual models, and reduce the effect of overfitting in a spirit of the bagging method [30].
%     - we choose Transformer [11], Bi-LSTM [18], and convolutional sequence to sequence [31] models to increase the diversity of ensemble models
% - Notes:
%     - Does ensemble prediction by averaging the predicted probability distribution of individual models. Straightforward to do this as outputs are discrete and network predictions are probability distributions

% 2. Ensemble Deep Neural Network Based Waveform-Driven Stress Model for Speech Synthesis (2016)
% https://link.springer.com/chapter/10.1007/978-3-319-43958-7_32
% % Google preview link: (section 2.3) https://books.google.co.uk/books?id=WFjYDAAAQBAJ&pg=PA271&lpg=PA271&dq=Ensemble+Deep+Neural+Network+Based+Waveform-Driven+Stress+Model+for+Speech+Synthesis&source=bl&ots=vYGwvZ6S1h&sig=ACfU3U0_q_JVE3eAUbkihfNMnewkB4kC9A&hl=en&sa=X&ved=2ahUKEwjfksGO_Nb6AhVrQkEAHYf1D_wQ6AF6BAgIEAM#v=onepage&q=Ensemble%20Deep%20Neural%20Network%20Based%20Waveform-Driven%20Stress%20Model%20for%20Speech%20Synthesis&f=false
% % Slides: http://www.specom2016.hte.hu/documents/1695342/3102158/05_01_toth_kiss_szaszak_nemeth.pdf
% - Section 2.3
%     The main goal of an ensemble model is to improve output performance by creating smaller,  more specialised networks whose aggregated knowledge may result in a better performance. This approach is especially useful when dealing with sparse signal modeling. IN the case of F0 modeling, training data with higher prosodic stress level is significantly less frequent in the database, therefore in a large, single model is likely to ignore the effect of these data elements, resultin gin a reduced performance of the whole model. To address this problem, an ensemble of four smaller feedforward networks was trained on different parts of the training database. The distinction was performed according to the prosodic stress levels. During testing, each ensemble member calculated its associated frames, again based on the prosodic stress levels. The end result was compiled from these frames. Each ensemble member model had the same 3 hidden layer architecture, but it contained only 1000 neurons in each hiden layer. The learning strategy, and the input-output values were also the same.
% - Snippets:
%     - This paper proposes a waveform based stress annotation technique. According to the stress classes, four feedforward deep neural networks (DNNs) were trained to model fundamental frequency (F0) of speech. During synthesis, stress labels are generated from the textual input and an ensemble of the four DNNs predict the F0 trajectories. 

% 3. Weighted Neural Network Ensemble Models for Speech Prosody Control (INTERSPEECH 2009)
% - Snippets: 
%     - Given prosody corpora of limited size, the statistical models that are applied in current TTS synthesis systems, like CART-, MARS-, HMM-, or ANN-based generation models, have one or more of the following disadvantages: their prediction accuracy is too low to achieve natural sounding prosody. Their generalization capability for input factor combinations that are not covered by the prosody corpora is not good enough. Or they are not robust enough against outliers of acoustic parameters due to errors in the segmentation, in the labeling, or in F0 extraction of the prosody corpora.
%     - For the ensemble construction of the prosody models, the author tested the W-SECA and the W-Bagging aggregation method. For W-Bagging, 6-fold cross validation was used instead of bootstrapping to obtain six different subsets of the training data. On each of these subsets, ANNs with eight different internal network structures, having one or two layers of hidden nodes and different number of nodes, were trained.
% - Notes: 
%     - Ensemble prediction (The prediction output of the ensemble is a linear combination of the prediction outputs of the individual models) of FF networks to model duration and F0 contours
%     - explored exponential, potential and mean weighting functions of the ensembles. Exponential weighting results in more robust error curves than potential weighting (and was chosen). 

% Anecdotally, we have observed performance differences between our research validation set and production test set, potentially due to factors such as shifts in length and linguistic distributions from the train set.

% Whiskers depict the 95\% confidence intervals, as converted from the corresponding odds ratios


==> tables/accuracy.tex <==
\begin{table}[htb]
    \renewcommand{\arraystretch}{1.5}%
    \resizebox{\columnwidth}{!}{%
        \begin{tabular}{l|c|c|c|c|c|c}
            \multicolumn{1}{c|}{\textbf{Accuracy (\%)}} & \multicolumn{1}{c|}{\textbf{M1}} & \multicolumn{1}{c|}{\textbf{M2}} & \multicolumn{1}{c|}{\textbf{GV}} & \multicolumn{1}{c|}{\textbf{WAV-F0}} & \multicolumn{1}{c|}{\textbf{AFP-F0}} & \multicolumn{1}{c}{\textbf{ORACLE}} \\ \hline
            \textbf{CONV-2} & 50.27 & 49.73 & 46.86 & 47.93 & 51.67 & \textbf{63.02*} \\ \hline
            \textbf{RNN-2} & 50.39 & 49.61 & 51.95 & 51.56 & 51.49 & \textbf{65.32*} \\ \hline
            \textbf{RNN-CONV} & 50.69 & 49.31 & 46.34 & \textbf{53.80*} & \textbf{55.18*} & \textbf{65.28*}
        \end{tabular}%
    }
    \caption{Accuracy of crowd wisdom, single models and ensemble selection. $^{\star}$ denotes accuracy rates that are statistically significantly above random chance.}
    \label{tab:accuracy}
\end{table}

==> tables/keywords.tex <==
\begin{table*}[htb]
    % \renewcommand{\arraystretch}{1}%
    \centering    
    % \resizebox{\columnwidth}{!}{%
        \begin{tabular}{l|c|c|c|c|c|c|c}
            \multicolumn{1}{l|}{\textbf{Keyword count}} & 
            \multicolumn{1}{l|}{\textbf{Expressiveness}} & 
            \multicolumn{1}{l|}{\textbf{Intonation}} & 
            \multicolumn{1}{l|}{\textbf{Emphasis}} & 
            \multicolumn{1}{l|}{\textbf{Clarity}} & 
            \multicolumn{1}{l|}{\textbf{Speed/pauses}} & 
            \multicolumn{1}{l|}{\textbf{Naturalness}} &             
            \multicolumn{1}{l}{\textbf{Other}} \\ \hline
            \textbf{CONV-2 (41)}  & 7 & 5 & 14 & 3 & 9 & 3 & 3\\ \hline
            \textbf{RNN-2 (68)} & 11 & 20 & 17 & 9 & 14 & 9 & 4 \\ \hline
            \textbf{RNN-CONV (97)} & 27 & 24 & 20 & 16 & 15 & 13 & 3
        \end{tabular}%
    % }
    \caption{Count of keywords tagged in free-text descriptions of the perceived diversity. The total number of comments received are in brackets next to each ensemble. Each comment has up to 3 keywords}
    \label{tab:keywords}
\end{table*}
